Context Aware Family Dynamics based Internet of Things Access Control Towards Better Child Safety

Today, children are increasingly connected to the Internet and consume content and services through various means. It has been a challenge for less tech-savvy parents to protect children from harmful content and services. Internet of Things (IoT) has made the situation much worse as IoT devices allow children to connect to the Internet in novel ways (e.g., connected refrigerators, TVs, and so on). In this paper, we propose mySafeHome, an approach which utilises family dynamics to provide a more natural, and intuitive access control mechanism to protect children from harmful content and services in the context of IoT. In mySafeHome, access control dynamically adapts based on the physical distance between family members. For example, a particular type of content can only be consumed, through TV, by children if the parents are in the same room (or hearing distance). mySafeHome allows parents to assess a given content by themselves. Our approach also aims to create granular levels of access control (e.g., block / limit certain content, features, services, on certain devices when the parents are not in the vicinity). We developed a prototype using OpenHAB and several smart home devices to demonstrate the proposed approach. We believe that our approach also facilitates the creation of better relationships between family members. A demo can be viewed here: http://safehome.technology/demo.

==> filtered_text.tex <==
 The system, currently designed, are device based and are using application level access control, but it is not feasible to install an application in all IoT devices considering the heterogeneity of IoTs. Considering the IoT architecture purposed by CISCO REFERENCE we can solve this problem going down a little at "Core Layer". Network access control (NAC) which is well established mechanism but need to be redesigned for this specific purpose. 

So, we have a possible way of controlling access, now the question is how we can detect the closeness/presence of a guardian near a child's device or an IoT device? Well, 

This can be done be either mathematical operations but then it will remain specific to the environment and for certain type of devices. So, w

, this method can be hosted on cloud as we did at the time of development to get better performance

The system also incorporates "allowed internet access" time schedule and guardians' google calendar and detect any on-going or scheduled meeting for the current time in order to better decision making and saving computational resources (it is obvious that the guardian is not at home). 

Most systems focused on controlling internet access of child device on application level which is specific to the mobile/tablets/computers only, so what about IoTs? How can we make sure that children are not exposed to bad side of internet using IoTs? Well, that is our work is all about.





bibs
%\begin{thebibliography}{1}
%
%\bibitem{IEEEhowto:kopka}
%H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
%
%\bibitem{IEEEhowto:kopka}
%H.~Singh et al, \emph{IoT based Smart Home Automation System using Sensor Node.}\hskip 1em plus
%  0.5em minus 0.4em\relax RAIT: 2018.
%  
%\bibitem{IEEEhowto:kopka}
%D.~Pal et al, \emph{Analyzing the Elderly Users' Adaptation of Smart-Home Services}\hskip 1em plus
%  0.5em minus 0.4em\relax IEEE: 2018.
%
%\bibitem{IEEEhowto:kopka}
%J.~Roux et al, \emph{RadIoT: Radio Communication Intrusion Detection for IoT - A Protocol Independent Approach}\hskip 1em plus
%  0.5em minus 0.4em\relax LAAS-CNRS: 2018.
%
%\bibitem{IEEEhowto:kopka}
%J.~Roux et al, \emph{Toward an Intrusion Detection Approach for IoT based Radio Communiaction Profiling}\hskip 1em plus
%  0.5em minus 0.4em\relax IEEE: 2018.
%
%\bibitem{IEEEhowto:kopka}
%Y.~Kashimoto et al, \emph{Low-cost Device-free Activity Recognition System with Energy Harvesting PIR and Door Sensors}\hskip 1em plus
%  0.5em minus 0.4em\relax ACM-CCS: 2016.
%
%\bibitem{IEEEhowto:kopka}
%P.~Kodeswaran et al, \emph{Demultiplexing Activities of Daily Living in IoT enabled Smarthomes}\hskip 1em plus
%  0.5em minus 0.4em\relax IEEE: 2016.
%
%\bibitem{IEEEhowto:kopka}
%C.~T.~Dang et al, \emph{Theodor: A Step Towards Smart Home Applications with Electronic Noses}\hskip 1em plus
%  0.5em minus 0.4em\relax IEEE: 2016.
%
%\bibitem{IEEEhowto:kopka}
%M.~Wang and W.~Qi, \emph{Harsh parenting and problematic Internet use in Chinese adolescents: Child emotional dysregulation as mediator and child forgiveness as moderator}\hskip 1em plus
%  0.5em minus 0.4em\relax Elsevier: 2017.
%
%\bibitem{IEEEhowto:kopka}
%S.~Nam and H.~Hwang, \emph{Consumers' Needs for Public Education and corporate Participation Regarding Child Internet Addiction: Based on the Risk Perception Attitude Framework}\hskip 1em plus
%  0.5em minus 0.4em\relax ---: 2018.
%
%\end{thebibliography}

